Bounding the Escape Time of a Linear Dynamical System over a Compact Semialgebraic Set

We study the Escape Problem for discrete-time linear dynamical systems over compact semialgebraic sets. We establish a uniform upper bound on the number of iterations it takes for every orbit of a rational matrix to escape a compact semialgebraic set defined over rational data. Our bound is doubly exponential in the ambient dimension, singly exponential in the degrees of the polynomials used to define the semialgebraic set, and singly exponential in the bitsize of the coefficients of these polynomials and the bitsize of the matrix entries. We show that our bound is tight by providing a matching lower bound.

==> tools.tex <==
\subsection{Mathematical tools}

Our characterisation of the complexity class $\EA$ requires two
sophisticated results from effective real algebraic geometry: Singly
exponential quantifier elimination and a doubly exponential bound on a
ball meeting all components of a semialgebraic set.  We use the
following singly exponential quantifier elimination result given in
\cite{BasuPollackRoy}.  For a historical overview on this type of result
see \cite[Chapter 14, Bibliographical Notes]{BasuPollackRoy}.

\begin{theorem}[{\cite[Theorem 14.16]{BasuPollackRoy}}]\label{Theorem: singly exponential quantifier elimination precise}
    Let $\mathcal{P}$ be a set of at most $s$ polynomials with integer coefficients,
    each of degree at most $d$, 
    in $k + n_1 + \dots + n_{\ell}$ variables.
    Let $\tau$ be a bound on the bitsize of the coefficients of all $P \in \mathcal{P}$.
    Let 
    \[
        \Phi_{\ell}(Y)
        =
        (Q_1 X_1).
        \dots 
        (Q_{\ell} X_{\ell}).
            \left(
                \Psi_0(Y, X_1,\dots, X_{\ell})
            \right),
    \]
    where $Q_j \in \{\exists, \forall\}$ are alternating blocks of quantifiers,
    be a formula over the language $\mathcal{L}$,
    all of whose atoms involve polynomials contained in $\mathcal{P}$.
    Assume that the size of the block of variables $Y$ is $k$ and 
    that the size of the block of variables $X_j$ is $n_j$. 

    Then there exists an equivalent quantifier-free formula
    \[ 
        \omega_0(Y)
        =
        \bigvee_{i = 1}^I \bigwedge_{j = 1}^{J_i} \bigvee_{m = 1}^{M_{i,j}}
            P_{i,j,m}(Y) \bowtie_{i,j,m} 0. 
    \]
    over 
    $\mathcal{L}$,
    where:
    \begin{enumerate}
        \item 
            $I \leq s^{(n_1 + 1)\cdot \dots \cdot (n_\ell + 1)(k + 1)} d^{O(n_1 \cdot \dots \cdot n_{\ell} \cdot k)}$.
        \item $J_i \leq s^{(n_1 + 1)\cdot \dots \cdot (n_\ell + 1)} d^{O(n_1 \cdot \dots \cdot n_{\ell})}$.
        \item $M_{i,j} \leq d^{O(n_1\cdot\dots\cdot n_\ell)}$.
        \item The degrees of the polynomials $P_{i,j,m}$ are bounded by $d^{O(n_1\cdot\dots\cdot n_{\ell})}$.
        \item The bitsize of the coefficients of the polynomials $P_{i,j,m}$ is bounded by $\tau d^{O(n_1\cdot\dots\cdot n_{\ell}\cdot k)}$.
    \end{enumerate}
\end{theorem}

Recall that a \emph{sign condition} on a family 
$\mathcal{P}$ 
of polynomials in $n$ variables is a mapping 
$\sigma \colon \mathcal{P} \to \{-1,0,1\}$.
The \emph{realisation} of a sign condition $\sigma$ in $\R^n$ is the set 
\[ 
    \operatorname{Reali}(\sigma) = \Set{X \in \R^n}{\forall P \in \mathcal{P}.\operatorname{sign}(P(X)) = \sigma(P)}.
\]
A sign condition $\sigma$ is called \emph{realisable} if its realisation is non-empty.
Equivalently, a sign condition is a formula over the language 
$\mathcal{L}$
involving only conjunctions.

The next theorem is due to Vorobjov \cite{Vorobjov84}.
See also \cite[Lemma 9]{GriorievVorobjov88} and \cite[Theorem 4]{BasuRoyRadiusBound}.

\begin{theorem}\label{Theorem: Basu-Roy radius bound}
    There exists an integer constant $\beta'$ with the following property:
    Let $\mathcal{P}$ be a set of $s$ polynomials with integer coefficients in $n$ variables of degree at most $d \geq 2$.
    Assume that the bit-size of the coefficients of each polynomial in $\mathcal{P}$ is at most $\tau$.
    Then there exists a ball centred at the origin of radius at most 
    \[
       2^{\tau d^{\beta' (n + 1)}}
    \]
    which intersects every connected component of every realisable sign condition on 
    $\mathcal{P}$
    in $\R^n$.
\end{theorem}

Our proof of $\EA$-completeness of CEP combines spectral methods with two well-known but nontrivial results on algebraic numbers.
We require a version of Kronecker's theorem on simultaneous Diophantine approximation.
See \cite[Corollary 3.1]{10.5555/2634074.2634101} for a proof.

\begin{theorem}
\label{Theorem: Kronecker}
    Let $(\lambda_1, \dots, \lambda_m)$ be complex algebraic numbers of modulus $1$.
    Consider the free Abelian group
    \[ 
        L = \Set{(n_1,\dots,n_m) \in \Z^m}{\lambda_1^{n_1}\cdot\dots\cdot \lambda_m^{n_m} = 1}.
    \]
    Let $(\beta_1,\dots,\beta_s)$ be a basis of $L$.
    Let $\mathbb{T}^m = \Set{(z_1,\dots,z_m) \in \C^m}{|z_j| = 1}$ denote the complex unit $m$-torus.
    Then the closure of the set 
    $\Set{(\lambda_1^k,\dots,\lambda_m^k) \in \mathbb{T}^m}{k \in \N}$
    is the set 
    $S = \Set{(z_1,\dots,z_m) \in \mathbb{T}^m}{\forall j\leq s. (z_1,\dots,z_m)^{\beta_j} = 1}$.

    Moreover, for all $\varepsilon > 0$ and all $(z_1,\dots,z_m) \in S$ 
    there exist infinitely many indexes $k$ such that 
    $|\lambda_j^k - z_j| < \varepsilon$
    for $j = 1,\dots,n$.
\end{theorem}

Moreover, the integer multiplicative relations between given complex algebraic numbers in the unit circle can be elicited in polynomial time.
For a proof see \cite{CaiLiptonZalcstein00, masser88}.
We assume the standard encoding of algebraic numbers, see \cite{Cohen} for details.

\begin{theorem}\label{Theorem: Masser}
    Let $(\lambda_1, \dots, \lambda_m)$ be complex algebraic numbers of modulus $1$.
    Consider the free Abelian group
    \[ 
        L = \Set{(n_1,\dots,n_m) \in \Z^m}{\lambda_1^{n_1}\cdot\dots\cdot \lambda_m^{n_m}}.
    \]
    Then one can compute in polynomial time a basis $(\beta_1,\dots,\beta_s) \in (\Z^m)^s$ for $L$.
    Moreover, the integer entries of the basis elements $\beta_j$ are bounded polynomially in the 
    size of the encodings of $\lambda_1,\dots,\lambda_m$.
\end{theorem}
